LUPET: Incorporating Hierarchical Information Path into Multilingual ASR

Toward high-performance multilingual automatic speech recognition (ASR), various types of linguistic information and model design have demonstrated their effectiveness independently. They include language identity (LID), phoneme information, language-specific processing modules, and cross-lingual self-supervised speech representation. It is expected that leveraging their benefits synergistically in a unified solution would further improve the overall system performance. This paper presents a novel design of a hierarchical information path, named LUPET, which sequentially encodes, from the shallow layers to deep layers, multiple aspects of linguistic and acoustic information at diverse granularity scales. The path starts from LID prediction, followed by acoustic unit discovery, phoneme sharing, and finally token recognition routed by a mixture-of-expert. ASR experiments are carried out on 10 languages in the Common Voice corpus. The results demonstrate the superior performance of LUPET as compared to the baseline systems. Most importantly, LUPET effectively mitigates the issue of performance compromise of high-resource languages with low-resource ones in the multilingual setting.

==> related_work.tex <==
\section{Related Work}
% previous research on LID/phoneme information 
Language identity (LID) is the commonly recognized feature that benefits multilingual ASR.  The most straightforward practice is to append LID embedding to the input acoustic features for model training [xx]. Though being highly effective, the LID information is assumed to be pre-known that may not be the case in practice. In [xx], LID prediction is performed via multi-task learning (MTL). To more explicitly utilizing LID, [xx] propose to classify spoken language by intermediate layers of encoder and self-condition the LID predictions on subsequent layers. By aligning LID label to the number of the decoding tokens, the connectionist temporal classification (CTC) loss for sequential labels can instead be used [xx] and demonstrates better results than utterance-level classification. Besides LID,  including phoneme recognition via MTL is also proved to help training multilingual ASR [xx]. UniSpeech [xx], a unified speech representation learning approach,  combines phonetic CTC learning with wav2vec2.0 [xx] via MTL, which shows great cross-lingual capabilities. The success of UniSpeech reflects the important role of phonetic information in multilingual scenarios.  

% previous research on MoE
Another line of research consider the architecture design. MoE is a very promising direction for multilingual ASR as different expert is intuitively expected to process different language-specific information.  Each expert is usually represented by a Feed-forward network (FFN). In [xx], the number of experts increase linearly with the language number when LID is used to select the expert.  Recent work [xx] presents a simple MoE implementation with a fixed number of experts that dynamically select top-2 experts conditioned on input frames performing well on the streaming Multilingual ASR. 

\begin{enumerate}[leftmargin=*]
    \item[(a)] \textit{Shallow} layers of the encoder are used to identify the LID information to condition the subsequent layers. % on which language is under transcription. 
    \item[(b)] With the benefits of SSL,  the input acoustic features are automatically quantized, clustered to discrete units, and then predicted from the \textit{Lower-middle} layer via MLM training.  
    \item[(c)] The learned acoustic units further facilitate the pronunciation learning of the \textit{Upper-middle} layer, thus utilizing the shared phoneme information across multiple languages. 
    \item[(d)] MoE including multiple feed-forward network (FFN) experts and a routing network are used to replace the FFN of \textit{Deep} layers. The input to the routing network is LID embedding from the shallow layer, which serves as a gate to guide hidden representations for language-specific processing.  
\end{enumerate}
